Accelerating Interactive Human-like Manipulation Learning with GPU-based Simulation and High-quality Demonstrations

Dexterous manipulation with anthropomorphic robot hands remains a challenging problem in robotics because of the high-dimensional state and action spaces and complex contacts. Nevertheless, skillful closed-loop manipulation is required to enable humanoid robots to operate in unstructured real-world environments. Reinforcement learning (RL) has traditionally imposed enormous interaction data requirements for optimizing such complex control problems. We introduce a new framework that leverages recent advances in GPU-based simulation along with the strength of imitation learning in guiding policy search towards promising behaviors to make RL training feasible in these domains. To this end, we present an immersive virtual reality teleoperation interface designed for interactive human-like manipulation on contact rich tasks and a suite of manipulation environments inspired by tasks of daily living. Finally, we demonstrate the complementary strengths of massively parallel RL and imitation learning, yielding robust and natural behaviors. Videos of trained policies, our source code, and the collected demonstration datasets are available at https://maltemosbach.github.io/interactive_ human_like_manipulation/.

==> framework_graph.tex <==

\usetikzlibrary{shapes.geometric, arrows, positioning}
% teleoperation nodes
% use this style instead for adding images of the devices
%\tikzstyle{devices} = [rectangle, rounded corners, minimum width=3cm, minimum height=1.3cm,text width=2.5cm, draw=black, fill=black!30]
\tikzstyle{devices} = [rectangle, rounded corners, minimum width=2.5cm, minimum height=1cm,text centered, draw=black, fill=black!30]
\tikzstyle{ros} = [rectangle, rounded corners, minimum width=2.5cm, minimum height=1cm,text centered, draw=black, fill=black!30]
\tikzstyle{sim} = [rectangle, rounded corners, minimum width=3cm, minimum height=6cm,text centered, text depth=5cm, draw=black, fill=black!15]

\tikzstyle{arrow} = [thick, ->, >=stealth]
\pgfdeclarelayer{bg}    % declare background layer
\pgfdeclarelayer{overlay}
\pgfsetlayers{bg, main, overlay}  % set the order of the layers (main is the standard layer)

\tikzset{
   teleop/.pic={
    \node (hmd) [devices] at (0, 4) {HMD};
    \node (tracker) [devices] at (0, 2.5) {VIVE tracker};
    \node (senseglove) [devices] at (0, -1.5) {SenseGlove};
    
    \node (viewer) [ros] at (6.5, 4) {VR Camera};
    \draw [arrow] (hmd) -- node[pos=0.65, anchor=north] {HMD pose} (viewer);
    
    \draw [arrow] (viewer.east) -- +(1, 0) -- +(1, 2) -| node[pos=0.28, anchor=north] {image} (hmd.north);
    
    \node (hand) [ros] at (1.5, 0.5) {Hand State};
    \draw [arrow] (tracker) -- node[pos=0.5, anchor=east] {wrist pose} (hand);
    \draw [arrow] (senseglove) -- node[pos=0.5, anchor=east] {finger angles} (hand);        

    \node (actor) [ros] at (6.5, 0.5) {Operator};
    \draw [arrow] (hand) -- node[pos=0.45, anchor=north] {hand state} (actor);
    \draw [arrow] (actor) -- node[pos=0.5, anchor=north west] {haptics} (senseglove.east);
 
    \begin{pgfonlayer}{bg}
        \node (sim) [sim] at (6.5, 2.5) {Simulation};
    \end{pgfonlayer}
    \begin{pgfonlayer}{overlay}
        \node[inner sep=0pt] (hmd) at (6.5, 2.25) {\includegraphics[width=.1 \textwidth]{images/components/sim_view.png}};
    \end{pgfonlayer}
   }
}

% version from thesis talk
\tikzset{
   teleop_old/.pic={
    \node (vive) [devices] at (0, 4) {VIVE devices};
    \node (senseglove) [devices] at (0, 0) {SenseGlove};
    \node (vr) [ros] at (11, 4) {OpenVR};
    
    \node (viewer) [ros] at (6.5, 4) {VR Camera};
    \draw [arrow] (vive) -- node[pos=0.65, anchor=north] {HMD pose} (viewer);
    
    \draw [arrow] (viewer) -- node[pos=0.5, anchor=north] {image} (vr);
    
    \node (hand) [ros] at (1.5, 2) {Hand State};
    \draw [arrow] (vive) -- node[pos=0.5, anchor=east] {wrist pose} (hand);
    \draw [arrow] (senseglove) -- node[pos=0.5, anchor=east] {finger angles} (hand);        

    \node (actor) [ros] at (6.5, 2) {Operator};
    \draw [arrow] (hand) -- node[pos=0.45, anchor=north] {hand state} (actor);
    \draw [arrow] (actor) -- node[pos=0.5, anchor=north west] {haptics} (senseglove.east);

    \begin{pgfonlayer}{bg}
        \node (sim) [sim] at (6.5, 2.5) {Simulation};
    \end{pgfonlayer}
    \begin{pgfonlayer}{overlay}
        \node[inner sep=0pt] (hmd) at (1.1, 4.3) {\includegraphics[width=.03\textwidth]{images/components/HTC-Vive-Pro2.png}};
        \node[inner sep=0pt] (hmd) at (1.1, 3.7) {\includegraphics[width=.04\textwidth]{images/components/tracker.png}};
        \node[inner sep=0pt] (hmd) at (1.1, 0) {\includegraphics[width=.04\textwidth]{images/components/SenseGlove-force-feedback.png}};
        \node[inner sep=0pt] (hmd) at (6.5, 0.5) {\includegraphics[width=.08 \textwidth]{images/components/sim_view.png}};
    \end{pgfonlayer}
   }
}

\scalebox{0.6}{%
    \begin{tikzpicture}
        \pic{teleop};
    \end{tikzpicture}%
}
